A Comprehensive Analysis of Three Microlensing Planet Candidates with the Planet/Binary Degeneracy

We present observations and analyses of three high-magnification microlensing events: KMT-2022-BLG-0954, KMT-2024-BLG-0697, and MOA-2024-BLG-018. All three exhibit the "Planet/Binary" degeneracy, with planetary solutions corresponding to mass ratios in the range $-3.7 < \log q < -2.2$, while the binary solutions yield $\log q > -2.0$. For KMT-2022-BLG-0954, we identify a previously unrecognized degeneracy among planetary solutions, involving different mass ratios and normalized source radii. In all three cases, single-lens binary-source models are excluded. Bayesian analyses suggest that the planetary solutions correspond to gas giants orbiting M/K dwarfs beyond the snow line, while KMT-2022-BLG-0954 also admits an alternative interpretation as a super-Earth orbiting a late-type M dwarf. The binary solutions imply a diverse set of systems, including M-dwarf pairs and M-dwarf--brown-dwarf binaries. A review of known events subject to the "Planet/Binary" degeneracy shows that in most cases the degeneracy cannot be resolved through follow-up high-resolution imaging, particularly in the presence of the newly identified degeneracy.

==> backup.tex <==


Figures \ref{KB220954_lc}, \ref{KB240697_lc}, and \ref{KB241170_lc} show the observed data around the peak region together with different models of KMT-2022-BLG-0954, KMT-2024-BLG-0697, and KMT-2024-BLG-1170, respectively. For KMT-2022-BLG-0954, the observed data exhibit a brightening followed by a dimming compared to the single-lens single-source (hereafter 1L1S) model \citep{Paczynski1986}. Such an asymmetric anomaly signal can potentially be produced by the orbital motion of Earth (parallax effect; \citealt{Gould1992, Gould2000, Gouldpies2004}), the orbital motion of the source star (xallarap effect; \citealt{Griest1992, HanGould1997}), the presence of a second lens (2L1S; \citealt{Shude1991, Andy1992}), or the presence of a second source (1L2S; \citealt{Gaudi1998}). However, the duration of the anomaly signal ($\sim$ 1 day) is significantly short compared to the overall event timescale ($\sim$ 45 days), which makes the parallax or xallarap explanations unlikely. As a consequence, the 1L1S model with higher-order effects can only improve the fit by $\Delta\chi^2 \sim 100$ with respect to the standard 1L1S model and can still not fit the anomaly signal well. Moreover, from Section \ref{subsection_kb220954}, we note that the 1L1S model with higher-order effects is disfavored by $\Delta\chi^2 > 600$ relative to the best-fit 2L1S model. Therefore, we exclude the 1L1S model with higher-order effects for KMT-2022-BLG-0954, while only 2L1S and 1L2S models are considered. For KMT-2024-BLG-0697 and KMT-2024-BLG-1170, the observed data show two bumps on the peak region, which can arise from either 2L1S or 1L2S. Thus, both 2L1S and 1L2S models should be investigated for these three events. In this Section, we perform the 2L1S analysis. 




As discussed in Section \ref{intro}, two-bump events may arise either from the source approaching two consecutive cusps of the diamond-shaped caustic in stellar binary models or from approaching the two off-axis cusps of the wedge-shaped caustic in planetary models. 
Among the three events, the observed data of KMT-2024-BLG-0697 and KMT-2024-BLG-1170 clearly exhibit two distinct bumps around the peak region, while the asymmetric peak of KMT-2022-BLG-0954 can also be interpreted as a superposition of two unresolved bumps and is ultimately found to be subject to the same type of degeneracy as the other two events, as will be shown later. 
Thus, a heuristic analysis of the multiplicity of models for such two-bump events helps in understanding the grid search results for the aforementioned events and ensures that no viable solutions are omitted during the modeling process. 



Since 2016, the advent of the Korea Microlensing Telescope Network (KMTNet; \citealt{KMT2016}) has revealed two types of degeneracies characterized by similar values of $s$ but different values of $q$. One is the ``Cannae/von Schlieffen'' degeneracy, which arises when a planetary caustic is crossed by a large source \citep{OB170173,2017_subprime}. In the ``Cannae'' model, the source fully envelops the planetary caustic, whereas in the ``von Schlieffen'' model, only one flank of the caustic is enveloped. The difference in $q$ between these models can be as large as a factor of three \citep{OB170173} to six \citep{2017_subprime}. The other is the ``caustic-chirality'' degeneracy \citep{OB170373,KB160212}, which occurs when the source passes over the planetary caustic. Although the two corresponding planetary models exhibit detectable differences in their anomalies, gaps in the data lead to the degeneracy.

In addition, two other types of degeneracies involve substantial differences in both $q$ and $s$. One arises when a large source crosses either a major-image caustic or a minor-image caustic \citep{OB110173,KB161107}. Unlike the degeneracies described above, the two corresponding models in this case predict different lens-source relative proper motions, $\mu_{\rm rel}$, and can therefore be resolved through late-time high-resolution imaging. The second type of degeneracy, which occurs in high-magnification (HM) events, was first identified by \cite{HanGaudi2008}, with \cite{OB110950} presenting the first realistic examples. In this case, a double-peaked anomaly can result from two cusp approaches to the central caustic, which may be produced either by a planetary system or a stellar binary. We refer to this as the ``Planet/Binary'' degeneracy. Because HM events are particularly sensitive to planetary perturbations \citep{Griest1998}, this degeneracy may introduce contamination into planetary statistical samples based on HM events.



%, which differs fundamentally from the classical $(\rho,q)$ continuous degeneracy described by \citet{Gaudi&Gould1997ApJ_continuous_degeneracy}. Unlike the classical degeneracy, this new degeneracy is discrete in nature, manifesting as distinct minima in parameter space rather than a continuous valley. While it shares the similar trend to the classical degeneracy, namely that larger $\rho$ corresponds to smaller $q$, the key distinction lies in the behavior of $s$: in the “Planet Finite” models, $s$ is closer to unity, leading to a larger caustic despite the smaller $q$, as shown in the top four panels of Figure \ref{KB220954_caustic}. We suspect that this degeneracy stems from the smooth, low-amplitude anomaly signal of this event. 


% It should be noted that the degeneracy between ``Planet'' model and ``Planet No FSE'' model is a new type of degeneracy, which is different from the well-known continuous degeneracy between $\rho$ and $q$ \citep{Gaudi&Gould1997ApJ_continuous_degeneracy} for two reasons: first, the new degeneracy is a discrete degeneracy instead of a continuous degeneracy; second, though the new degeneracy has the same trend as the previous degeneracy that larger $\rho$ corresponds to smaller $q$, but the fact that $s$ is also closer to 1 produces even larger caustic for the model with larger $\rho$, as shown in Figure \ref{KB220954_caustic} (top four panels). 
% We attribute/suspect the origin of this degeneracy to/from the very smooth anomaly signal of this event. 

% However, although having the lowest $\chi^2$, the `Close Planet'' and Wide Planet'' models are finally rejected by the unlikely small $\murel$ derived in Section \ref{CMD}. 
% Following the $\murel$ distribution of observed planetary microlensing events \citep{MASADA}, \cite{2019_subprime} showed that the fraction of events with relative proper motions lower than a given $\murel \ll \sigma_{\mu}$ is 
% \begin{equation}\label{eqn:probmu}
% p(\leq\murel) \rightarrow \frac{\murel^2}{4\sigma_{\mu}^2} \rightarrow 2.8 \times 10^{-2}\biggl(\frac{\murel}{1\,{\rm mas\,yr^{-1}}}\biggr)^2,
% \end{equation}
% where we adopt $\sigma_{\mu} = 3.0\,{\rm mas\,yr^{-1}}$ for the relative proper motion dispersion. 
% For example, $p(\leq 1\,{\rm mas\,yr^{-1}}) = 2.8\%$ and $p(\leq 0.7\,{\rm mas\,yr^{-1}}) = 1.4\%$. 
% However, Table \ref{table:CMD} shows that the inferred relative proper motion for the `Close Planet'' and Wide Planet'' models is $\murel = 0.69 \pm 0.04 \,{\rm mas\,yr^{-1}}$, which is thus of very low probability. 
% Thus, we reject the `Close Planet'' and Wide Planet'' models and take the Close Planet No FSE'' and Wide Planet No FSE'' models as the only possible models with planetary mass ratios. 

% Now the `Close Binary D→A'' and Wide Binary D→A'' models provide the best fit to the data, while the Close Planet No FSE'', Wide Planet No FSE'', Close Binary A→B'', Wide Binary A→B'', Wide Binary B→C'', and Wide Binary C→D'' models are disfavoured by $\Delta\chi^2$ = 4.3, 4.3, 6.1, 5.3, 9.6, and 11.0, respectively. 
% Due to the small $\Delta\chi^2$ between different models, all remaining eight models cannot be rejected, while the planetary and preferred stellar binary model pairs are marked in boldface in Table \ref{KB220954_parm_2L1Sstatic}. 
% The $\te$ for the `Wide Binary B→C'' and Wide Binary C→D'' models are significantly longer than other models, which is due to the secondary lens dominated nature of these two models ($q > 1$). 
% 
% 
% Despite yielding the lowest $\chi^2$, the ``Close Planet Finite'' and ``Wide Planet Finite'' models are finally rejected (\HL{may need to change to highly unlikely instead of rejected}) due to their unlikely small inferred relative proper motion, as derived in Section \ref{CMD}. 
Despite yielding the lowest $\chi^2$, the ``Close Planet Finite'' and ``Wide Planet Finite'' models are considered statistically disfavored due to their unusually small inferred relative proper motion, as derived in Section \ref{CMD}. 
% I also have a stronger statement version: 
% Despite yielding the lowest $\chi^2$, the ``Close Planet Finite'' and ``Wide Planet Finite'' models are considered unlikely due to their unusually small inferred relative proper motion, as derived in Section \ref{CMD}.
%Following the $\murel$ distribution of observed planetary microlensing events \citep{MASADA}, \cite{2019_subprime} showed that the fraction of events with relative proper motions lower than a given $\murel \ll \sigma_{\mu}$ is 
%\begin{equation}\label{eqn:probmu}
%p(\leq\murel) \rightarrow \frac{\murel^2}{4\sigma_{\mu}^2} \rightarrow 2.8 \times 10^{-2}\biggl(\frac{\murel}{1\,{\rm mas\,yr^{-1}}}\biggr)^2,
%\end{equation}
%where we adopt $\sigma_{\mu} = 3.0\,{\rm mas\,yr^{-1}}$ for the relative proper motion dispersion. 
%This implies, for example, a probability of only $2.8\%$ for $\murel \leq 1\,{\rm mas\,yr^{-1}}$, and $1.4\%$ for $\murel \leq 0.7\,{\rm mas\,yr^{-1}}$. 
%As shown in Table \ref{table_CMD_kb220954}, both the ``Close Planet Finite'' and ``Wide Planet Finite'' models yield $\murel = 0.69 \pm 0.04 \,{\rm mas\,yr^{-1}}$, which is thus of very low probability. However, we retain these two models for further analysis in the following sections.


% Among the eight retained models, the ``Close Binary D→A'' and ``Wide Binary D→A'' models provide the best fit to the data, while the ``Close Planet No FSE'', ``Wide Planet No FSE'', ``Close Binary A→B'', ``Wide Binary A→B'', ``Wide Binary B→C'', and ``Wide Binary C→D'' models are disfavoured by $\Delta\chi^2$ = 4.3, 4.3, 6.1, 5.3, 9.6, and 11.0, respectively. 
% Given the relatively small $\Delta\chi^2$ between different models, none of these eight models can be decisively ruled out, while the pairs of planetary and favored stellar binary models are highlighted in bold in Table \ref{KB220954_parm_2L1Sstatic}. 
% The ``Wide Binary B→C'' and ``Wide Binary C→D'' models exhibit significantly longer $\te$ than other models, which is due to the much more massive secondary lens of these two models ($q \gg 1$). 
% % large te for the two wide solutions are due to our convention of allowing q to be >1

% dding parallax cannot imporve the fit, and contrdiact delta chi2 between different data set. 


Similar to \eventa, two wide binary models, ``Wide Binary CD'' and ``Wide Binary DA'', exhibit significantly longer $\te$ due to their much more massive secondary lens ($q \gg 1$). 
, grouped into three categories: the two planetary models, the two close binary models, and the four wide binary models. 
Unlike \eventa, $\rho$ is well constrained for all eight models of \eventb. 
This is attributed to the more complete observational coverage and the stronger anomaly signal compared to \eventa, the latter resulting from a closer source trajectory and larger caustics. 
% caustic figure, fse
The ``Wide Binary AB'' model provides the best fit to the data, while the ``Close Binary AB'', ``Close Planet'', ``Wide Planet'', ``Close Binary BC'', ``Wide Binary BC'', ``Wide Binary CD'', and ``Wide Binary DA'' models are disfavoured by $\Delta\chi^2$ = 0.5, 8.0, 7.9, 68.0, 66.9, 87.0, and 77.7, respectively. 
% lc, systematic residual, wide are similar, combined the large dchi2 and systematic residual , we exculde
Figure \ref{KB240697_lc} displays the model light curves together with the residuals of the three ``Close'' models and the cumulative distribution of $\chi^2$ differences for the ``Close Binary AB'' and ``Close Binary BC'' models compared to the ‘Close Planet’ model. 
We find that the ``Close Binary BC'' model cannot well fit the interval between the two bumps and the rising part of the peak, with the main $\chi^2$ differences contributed by the KMTC19 ($I$) and LCOS ($I$) data. 
% lcos contributes dchi2=8, the remaining is from KMTC19
The ``Wide Binary BC'', ``Wide Binary CD'', and ``Wide Binary DA'' models show similar deficiencies. 
Given their large $\Delta\chi^2$ compared to the best-fit model and the presence of systematic residuals, we exclude the ``Close Binary BC'', ``Wide Binary BC'', ``Wide Binary CD'', and ``Wide Binary DA'' models, and only investigate the two ``Planet'' models and the two ``Binary AB'' models in the following analysis. 
% , which are highlighted in bold in Table \ref{KB240697_parm_2L1Sstatic}. 
We note that although several models are excluded, the ``Planet/Binary'' degeneracy persists for \eventb. 

% The eight minima with stellar binary mass ratios are further divided into close ($s<1$) and wide ($s>1$) configurations through the ``close/wide'' degeneracy, and there are a total of four distinct orientations of the source trajectory (i.e., four groups of $\alpha$ values) identified. 
% Among the four close minima, the two minima labeled with ``Counterpart'' are intrinsically identical to the other two orientations with $\log q > 0$, while the four wide minima are non-redundant to each other, as Section \ref{subsection_2L1S_Preamble} indicates. 
% This leaves six unique stellar binary models, which correspond exactly to the expected multiplicity of models for two-bump events and are labeled as ``Close Binary D→A'', ``Close Binary A→B'', ``Wide Binary D→A'', ``Wide Binary A→B'', ``Wide Binary B→C'', and ``Wide Binary C→D'', reflecting the order in which the source trajectories pass the cusps of the diamond-shaped caustic. 

% The four minima with planetary mass ratios deviate from the standard expectation of two planetary models for two-bump events. 
% In addition to the ``close/wide'' degeneracy, on each side of $s=1$, we find two minima: one with a smaller $q$ and $s$ near unity, the other with a larger $q$ and $s$ more deviated from unity. 
% Our subsequent analysis reveals that $\rho$ cannot be well constrained for the latter pair of minima. 
% Accordingly, we designate the four models as ``Close Planet'', ``Close Planet No FSE'', ``Wide Planet'', ``Wide Planet No FSE'', where ``No FSE'' indicates the finite-source effect is marginally detected. 














% \begin{table*}
% %[htb]
%     \renewcommand\arraystretch{1.25}
%     \centering
%     \caption{2L1S static models for KMT-2024-BLG-0697}
%     %\caption{Lensing Parameters for KMT-2022-BLG-0440}
    
%     \resizebox{\textwidth}{!}{
    
%     \begin{tabular}{c|c c c c|c c c c c c}
%     \hline
%     \hline
%     \multirow{2}{*}{Parameters} &  \multicolumn{4}{c|}{Close} & \multicolumn{6}{c}{Wide} \\ %\cline{2-7} 
%     %\hline
%      %&
%      %$u_0>0$ & $u_0<0$ & $u_0>0$ & $u_0<0$ \\
%       & \multicolumn{1}{c}{\textbf{Planetary}} & \multicolumn{1}{c}{\textbf{Binary1}} & Binary2 & Binary2 & \multicolumn{1}{c}{\textbf{Planetary}} & \multicolumn{1}{c}{\textbf{Binary1}} & Binary2 & Binary3 & Binary4 & Binary4 \\
%     \hline
%     $\chi^2$/dof  
%     & $2637.9/2638$ 
%     & $2737.7/2638$ 
%     & $2712.6/2638$ 
%     & $2712.6/2638$ 
    
%     & $2638.3/2638$ 
%     & $2729.0/2638$ 
%     & $2712.7/2638$
%     & $2729.0/2638$ 
%     & $2712.7/2638$ 
%     & $2729.0/2638$ \\
    
%     \hline
%     $t_{0} - 10425$ (${\rm HJD}^{\prime}$) 
%     & $0.7413 \pm 0.0009$ 
%     & $0.5423 \pm 0.0002$ 
%     & $0.4353 \pm 0.0089$ 
%     & $0.4334 \pm 0.0085$     
    
%     & $0.5395 \pm 0.0004$ 
%     & $0.5424 \pm 0.0002$ 
%     & $0.4334 \pm 0.0085$
%     & $0.5424 \pm 0.0002$ 
%     & $0.4334 \pm 0.0085$ 
%     & $0.4334 \pm 0.0085$ \\  
    
%     $u_{0} (10^{-3})$ 
%     & $0.0073 \pm 0.0006$ 
%     & $4.2 \pm 0.1$ 
%     & $1.5 \pm 0.2$ 
    
%     & $4.1 \pm 0.1$ 
%     & $4.2 \pm 0.2$ 
%     & $1.5 \pm 0.1$
%     & $4.2 \pm 0.2$ 
%     & $1.5 \pm 0.1$ \\
    
%     $\te$ (days) & $41.08 \pm 1.37$ & $40.03 \pm 1.35$ & $41.97 \pm 1.54$ & $41.29 \pm 1.41$ & $40.06 \pm 1.45$ & $42.62 \pm 1.53$ \\
    
%     $\rho (10^{-3})$ & $<1.032$ & $0.881 \pm 0.055$ & $<0.891$ & $<1.028$ & $0.904 \pm 0.098$ & $<0.803$ \\
%     $\alpha$ (degree) & $298.83 \pm 0.43$ & $296.34 \pm 0.28$ & $ 43.89 \pm 1.05$ & $298.77 \pm 0.41$ & $296.03 \pm 0.51$ & $ 43.89 \pm 0.97$ \\
%     $s$ & $0.6359 \pm 0.0195$ & $0.9933 \pm 0.0004$ & $0.1112 \pm 0.0075$ & $1.5799 \pm 0.0463$ & $1.0114 \pm 0.0004$ & $9.3771 \pm 0.6409$ \\
%     $q (10^{-4})$ & $0.880 \pm 0.123$ & $0.176 \pm 0.009$ & $325.0 \pm 48.1$ & $0.876 \pm 0.116$ & $0.180 \pm 0.009$ & $339.7 \pm 48.9$\\ 
%     $\log q$ & $-4.060 \pm 0.061$ & $-4.754 \pm 0.023$ & $-1.492 \pm 0.061$ & $-4.061 \pm 0.058$ & $-4.744 \pm 0.023$ & $-1.473 \pm 0.061$ 
%     \\
%     $I_{\rm S, OGLE}$ 
%     & $20.172 \pm 0.037$ & $20.142 \pm 0.037$ & $20.196 \pm 0.041$ 
%     & $20.167 \pm 0.037$ & $20.139 \pm 0.039$ & $20.174 \pm 0.040$\\

%     \iffalse
%     $V_{\rm S, OGLE}$ 
%     & $21.983 \pm 0.037$ & $21.951 \pm 0.037$ & $22.007 \pm 0.041$ 
%     & $21.988 \pm 0.038$ & $21.953 \pm 0.040$ & $22.006 \pm 0.040$\\
    
%     $I_{\rm B, OGLE}$ 
%     & $18.236 \pm 0.052$ & $18.241 \pm 0.052$ & $18.232 \pm 0.052$ 
%     & $18.235 \pm 0.052$ & $18.241 \pm 0.052$ & $18.232 \pm 0.052$\\
    
%     $V_{\rm B, OGLE}$ 
%     & $19.999 \pm 0.103$ & $20.004 \pm 0.104$ & $19.995 \pm 0.103$ 
%     & $19.998 \pm 0.103$ & $20.004 \pm 0.104$ & $19.995 \pm 0.103$\\
%     \fi
    
%     \hline
%     \hline
%     \end{tabular}

%     }
    
%     \begin{tablenotes}
%         \centering
%         \item{NOTE. } 
%         ${\rm HJD}^{\prime} = {\rm HJD} - 2450000$. 
%         $t_0$ and $u_0$ take the magnification center as the origin, which is the mass center when $s<1$ and ? when $s>1$. 
%     \end{tablenotes}
%     %\tablecomments{The upper limits on $\rho$ are at $3\sigma$.}The upper limit on $\rho$ is $3\sigma$. 
%     \label{KB240697_parm_2L1Sstatic}
% \end{table*}







% \begin{table*}
% %[htb]
%     % \centering
%     % \renewcommand{\arraystretch}{1.4}
%     \renewcommand\arraystretch{1.25}
%     \centering
%     \caption{2L1S static models for KMT-2024-BLG-0697}
%     %\caption{Lensing Parameters for KMT-2022-BLG-0440}
    
%     \resizebox{\textwidth}{!}{
    
%     \begin{tabular}{c|c c c|c c c c c}
%     \hline
%     \hline
%     \multirow{2}{*}{Parameters} &  \multicolumn{3}{c|}{Close} & \multicolumn{5}{c}{Wide} \\ %\cline{2-7} 
%     %\hline
%      %&
%      %$u_0>0$ & $u_0<0$ & $u_0>0$ & $u_0<0$ \\
%       & \multicolumn{1}{c}{\textbf{Planetary}} & \multicolumn{1}{c}{\textbf{Binary1}} & Binary2 & \multicolumn{1}{c}{\textbf{Planetary}} & \multicolumn{1}{c}{\textbf{Binary1}} & Binary2 & Binary3 & Binary4 \\
%     \hline
%     $\chi^2$/dof  
%     & $2637.9/2638$ 
%     & $2737.7/2638$ 
%     & $2712.6/2638$ 
    
%     & $2638.3/2638$ 
%     & $2729.0/2638$ 
%     & $2712.7/2638$
%     & $2729.0/2638$ 
%     & $2712.7/2638$ \\
    
%     \hline
%     $t_{0} - 10425$ (${\rm HJD}^{\prime}$) 
%     & $0.7413 \pm 0.0009$ 
%     & $0.5423 \pm 0.0002$ 
%     & $0.4353 \pm 0.0089$ 
    
%     & $0.5395 \pm 0.0004$ 
%     & $0.5424 \pm 0.0002$ 
%     & $0.4334 \pm 0.0085$
%     & $0.5424 \pm 0.0002$ 
%     & $0.4334 \pm 0.0085$ \\  
    
%     $u_{0} (10^{-3})$ 
%     & $0.0073 \pm 0.0006$ 
%     & $4.2 \pm 0.1$ 
%     & $1.5 \pm 0.2$ 
    
%     & $4.1 \pm 0.1$ 
%     & $4.2 \pm 0.2$ 
%     & $1.5 \pm 0.1$
%     & $4.2 \pm 0.2$ 
%     & $1.5 \pm 0.1$ \\
    
%     $\te$ (days) & $41.08 \pm 1.37$ & $40.03 \pm 1.35$ & $41.97 \pm 1.54$ & $41.29 \pm 1.41$ & $40.06 \pm 1.45$ & $42.62 \pm 1.53$ \\
    
%     $\rho (10^{-3})$ & $<1.032$ & $0.881 \pm 0.055$ & $<0.891$ & $<1.028$ & $0.904 \pm 0.098$ & $<0.803$ \\
%     $\alpha$ (degree) & $298.83 \pm 0.43$ & $296.34 \pm 0.28$ & $ 43.89 \pm 1.05$ & $298.77 \pm 0.41$ & $296.03 \pm 0.51$ & $ 43.89 \pm 0.97$ \\
%     $s$ & $0.6359 \pm 0.0195$ & $0.9933 \pm 0.0004$ & $0.1112 \pm 0.0075$ & $1.5799 \pm 0.0463$ & $1.0114 \pm 0.0004$ & $9.3771 \pm 0.6409$ \\
%     $q (10^{-4})$ & $0.880 \pm 0.123$ & $0.176 \pm 0.009$ & $325.0 \pm 48.1$ & $0.876 \pm 0.116$ & $0.180 \pm 0.009$ & $339.7 \pm 48.9$\\ 
%     $\log q$ & $-4.060 \pm 0.061$ & $-4.754 \pm 0.023$ & $-1.492 \pm 0.061$ & $-4.061 \pm 0.058$ & $-4.744 \pm 0.023$ & $-1.473 \pm 0.061$ 
%     \\
%     $I_{\rm S, OGLE}$ 
%     & $20.172 \pm 0.037$ & $20.142 \pm 0.037$ & $20.196 \pm 0.041$ 
%     & $20.167 \pm 0.037$ & $20.139 \pm 0.039$ & $20.174 \pm 0.040$\\

%     \iffalse
%     $V_{\rm S, OGLE}$ 
%     & $21.983 \pm 0.037$ & $21.951 \pm 0.037$ & $22.007 \pm 0.041$ 
%     & $21.988 \pm 0.038$ & $21.953 \pm 0.040$ & $22.006 \pm 0.040$\\
    
%     $I_{\rm B, OGLE}$ 
%     & $18.236 \pm 0.052$ & $18.241 \pm 0.052$ & $18.232 \pm 0.052$ 
%     & $18.235 \pm 0.052$ & $18.241 \pm 0.052$ & $18.232 \pm 0.052$\\
    
%     $V_{\rm B, OGLE}$ 
%     & $19.999 \pm 0.103$ & $20.004 \pm 0.104$ & $19.995 \pm 0.103$ 
%     & $19.998 \pm 0.103$ & $20.004 \pm 0.104$ & $19.995 \pm 0.103$\\
%     \fi
    
%     \hline
%     \hline
%     \end{tabular}

%     }
    
%     \begin{tablenotes}
%         \centering
%         \item{NOTE. } 
%         ${\rm HJD}^{\prime} = {\rm HJD} - 2450000$. 
%         $t_0$ and $u_0$ take the magnification center as the origin, which is the mass center when $s<1$ and ? when $s>1$. 
%     \end{tablenotes}
%     %\tablecomments{The upper limits on $\rho$ are at $3\sigma$.}The upper limit on $\rho$ is $3\sigma$. 
%     \label{KB240697_parm_2L1Sstatic}
% \end{table*}



% \begin{figure}
%     %\centering
%     \includegraphics[width=0.47\textwidth]{Fig/KB220954_publish_cmd.png}
%     \caption{Color-magnitude diagram (CMD) of KMT-2022-BLG-0954.
%     error bar is smaller than marker size. only plot one source position, because source positions of three solutions are within one sigma and the position difference is much smaller than marker size. }
% \label{KB220954_cmd}
% %\end{figure*}
% \end{figure}




% %\begin{figure*}
% \begin{figure}
%     %\centering
%     \includegraphics[width=0.47\textwidth]{Fig/KB240697_publish_cmd.png}
%     \caption{Color-magnitude diagram (CMD) of KMT-2024-BLG-0697, which is constructed by the field stars (black points) within $2.5^{\prime}$ centered on the source position using the OGLE-III star catalog \citep{OGLEIII}. The red asterisk represents the centroid of the red clump (RC), the blue dot indicates the source of the 2L1S model, and the yellow dot shows the blended light of the OGLE-III baseline object. The magenta and brown dots represent the second source of the 1L2S models with and without the color-color constraint (i.e., the third and first solutions in Table \ref{parm_1L2S}). The green points represent the HST CMD of \citet{HSTCMD} whose RC has been matched to that of OGLE-III. The blue line indicates the blue boundary of the bulge main-sequence stars derived from stellar isochrones with [M/H] = $-1.0$ and age $>9$ Gyr.}
% \label{KB240697_cmd}
% %\end{figure*}
% \end{figure}




% \begin{figure}
%     %\centering
%     \includegraphics[width=0.47\textwidth]{Fig/KB241170_publish_cmd.png}
%     \caption{Color-magnitude diagram (CMD) of KMT-2024-BLG-1170. }
% \label{KB241170_cmd}
% %\end{figure*}
% \end{figure}

%and the fraction of events for disk lenses is lower due to higher 

% \begin{table*}
%     \caption{CMD parameters, source properties and derived $\thetae$ and $\murel$ for the three events}
%     \centering
%     \renewcommand{\arraystretch}{1.4}
%     \begin{tabular}{c | c c c}
%     \hline \hline 
%     Event & KMT-2022-BLG-0954 & KMT-2024-BLG-0697 & KMT-2024-BLG-1170 \\
%     \hline 
%     $(V - I)_{\rm RC}$    & $1.830 \pm 0.007$  & $2.508 \pm 0.016$  & $1.973 \pm 0.009$ \\
%     $I_{\rm RC}$          & $15.353 \pm 0.020$ & $17.050 \pm 0.063$ & $15.740 \pm 0.038$\\
%     \hline 
%     $(V - I)_{\rm RC, 0}$ & $1.06 \pm 0.03$    & $1.06 \pm 0.03$    & $1.06 \pm 0.03$   \\
%     $I_{\rm RC, 0}$       & $14.38 \pm 0.04$   & $14.35 \pm 0.04$   & $14.60 \pm 0.04$  \\
%     \hline 


    
%     $(V - I)_{\rm S}$     & $1.627 \pm 0.006$  & $2.234 \pm 0.032$  & $1.721 \pm 0.094$\\
%      %\multirow{2}{*}{$I_{\rm S}$} 

%     $I_{\rm S}$   & $20.33 \pm 0.02$ for Planet & $21.49 \pm 0.09$ for Planet & $19.70 \pm 0.04$ for Planet \\ 
%                   & $20.35 \pm 0.02$ for Planet No FSE & $21.42 \pm 0.10$ for Binary A→B & $19.52 \pm 0.04$ for Binary C→D \\
%                   & $20.34 \pm 0.02$ for Binary D→A & & \\
%     \hline         


    
%     $(V - I)_{\rm S,0}$ & $0.86 \pm 0.03$ & $0.79 \pm 0.05$ & $0.81 \pm 0.10$ \\
    
%     $I_{\rm S,0}$ 
%     & $19.36 \pm 0.05$ for Planet        & $18.79 \pm 0.12$ for Planet     & $18.56 \pm 0.07$ for Planet \\ 
%     & $19.38 \pm 0.05$ for Planet No FSE & $18.72 \pm 0.12$ for Binary A→B & $18.38 \pm 0.07$ for Binary C→D \\
%     & $19.37 \pm 0.05$ for Binary D→A    & & \\
%     \hline        


    
%     $\theta_*$ ($\mu$as) 
%     & $0.49 \pm 0.02$ for Planet        & $0.60 \pm 0.04$ for Planet     & $0.68 \pm 0.06$ for Planet \\
%     & $0.49 \pm 0.02$ for Planet No FSE & $0.62 \pm 0.04$ for Binary A→B & $0.74 \pm 0.07$ for Binary C→D \\
%     & $0.49 \pm 0.02$ for Binary D→A    & & \\
    
%     \hline                      
%     $\thetae$ (mas) 
%     & $0.084 \pm 0.005$ for Planet & $0.24 \pm 0.03$ for Planet     & $>0.041$ for Planet \\
%     & $>0.095$ for Planet No FSE   & $0.28 \pm 0.04$ for Binary A→B & $>0.052/0.115$ for Binary C→D Close/Wide \\
%     & $>0.078/0.093$ for Binary D→A Close/Wide   & & \\
    
%     \hline                      
%     $\murel$ (${\rm mas\,yr^{-1}}$) 
%     & $0.69 \pm 0.04$ for Planet & $5.8 \pm 0.8$ for Planet     & $>1.06$ for Planet \\
%     & $>0.76$ for Planet No FSE  & $7.1 \pm 1.2$ for Binary A→B & $>1.52/1.53$ for Binary C→D Close/Wide \\
%     & $>0.63/0.68$ for Binary D→A Close/Wide & & \\
    
%     \hline \hline
%     \end{tabular}
%     \begin{tablenotes}
%       %\centering
%       \item{NOTE. }
%       %\item[1]  
%       The lower limits on $\thetae$ and $\murel$ are $3\sigma$. $[(V - I),~I]_{\rm RC}$ and $[(V - I),~I]_{\rm S}$ of KMT-2024-BLG-0697 are not in OGLE-III magnitude scale. (for 220954, the Planet solution is rejected because of too small murel. So we need to compare between the Planet No FSE and Binary solutions, thus more MCMC need to be run to precisely determine the 3 sigma upper limit for rho (Done).  )
%       %$(V - I)_{\rm RC}$ and $I_{\rm RC}$ of KMT-2024-BLG-0697 are not in OGLE-III magnitude scale. 
%     \end{tablenotes}
%     \label{table:CMD}
% \end{table*}

 The reddening and extinction for the red clump toward each event are then computed as 
\begin{equation}\label{equ:extinction1}
    (E(V - I), A_I) = (V-I, I)_{\rm RC} - (V-I, I)_{\rm RC,0}. 
\end{equation}


\iffalse
\begin{table*}
    \caption{CMD parameters, source properties and derived $\thetae$ and $\murel$ for \event}
    \renewcommand{\arraystretch}{1.4}
    \begin{tabular}{c|c c c c}
    \hline \hline 
    Solution & Close Central ($u_0 > 0$) & Close Central ($u_0 < 0$) & Wide Central ($u_0 > 0$) & Wide Central ($u_0 < 0$) \\
    \hline
    $(V - I)_{\rm RC}$ & $2.143 \pm 0.007$ & $\gets$ & $\gets$ & $\gets$ \\
    $I_{\rm RC}$ & $15.920 \pm 0.022$ & $\gets$ & $\gets$ & $\gets$ \\
    $(V - I)_{\rm RC, 0}$ & $1.06 \pm 0.03$ & $\gets$ & $\gets$ & $\gets$ \\
    $I_{\rm RC, 0}$ & $14.53 \pm 0.04$ & $\gets$ & $\gets$ & $\gets$ \\
    $(V - I)_{\rm S}$ & $1.820 \pm 0.003$ & $\gets$ & $\gets$ & $\gets$  \\
    $I_{\rm S}$ & $20.135 \pm 0.035$ & $20.136 \pm 0.033$ & $20.151 \pm 0.038$ & $20.132 \pm 0.036$ \\ 
    $(V - I)_{\rm S,0}$ & $0.74 \pm 0.03$ & $\gets$ & $\gets$ & $\gets$ \\
    $I_{\rm S,0}$ & $19.02 \pm 0.06$ & $19.04 \pm 0.06$ & $19.01 \pm 0.06$ & $19.02 \pm 0.06$ \\ 
    $\theta_*$ ($\mu$as) & $0.516 \pm 0.022$ & $0.512 \pm 0.021$ & $0.519 \pm 0.022$ & $0.516 \pm 0.022$ \\
    $\thetae$ (mas) & $>0.42$ & $>0.43$ & $>0.41$ & $>0.47$ \\ 
    $\murel$ (${\rm mas\,yr^{-1}}$) & $>3.9$ & $>4.0$ & $>3.8$ & $>4.3$ \\ 
    \hline \hline
    \end{tabular}
    \begin{tablenotes}
        \centering
        \item{NOTE.} The lower limits on $\thetae$ and $\murel$ are $3\sigma$.
    \end{tablenotes}
    \label{table:source}
\end{table*}
\fi


% \begin{table*}
% %[htb]
%     \renewcommand\arraystretch{1.25}
%     \centering
%     \caption{1L2S models for \event}
%     \begin{tabular}{c|c c c c}
%     \hline
%     \hline
%     color argument? & $\times$ & $\surd$ & $\times$ & $\surd$ \\
%     color-color constraint? & $\times$ & $\times$ & $\surd$ & $\surd$ \\
%     \hline    
%     $\chi^2_{\rm total}$/dof 
%     & $2627.0/2635$ & $2646.2/2635$ & $2628.9/2635$ & $2674.5/2635$\\ 
%     \hline
%     $t_{0,1} - 9703$ (${\rm HJD}^{\prime}$) 
%     & $0.5351 \pm 0.0008$ & $0.5356 \pm 0.0007$ & $0.5349 \pm 0.0008$ & $0.5364 \pm 0.0007$\\
%     $t_{0,2} - 9703$ (${\rm HJD}^{\prime}$) 
%     & $0.6235 \pm 0.0013$ & $0.6240 \pm 0.0012$ & $0.6234 \pm 0.0013$ & $0.6254 \pm 0.0011$\\
%     $u_{0,1} (10^{-3})$  
%     & $4.1 \pm 0.2$ & $4.1 \pm 0.2$ & $4.1 \pm 0.2$ & $4.1 \pm 0.2$ \\
%     $u_{0,2} (10^{-3})$  
%     & $1.4 \pm 0.3$ & $1.3 \pm 0.5$ & $1.5 \pm 0.2$ & $0.7 \pm 0.6$ \\
%     $\te$ (days) 
%     & $42.05 \pm 1.52$ & $41.38 \pm 1.35$ & $41.97 \pm 1.49$ & $41.80 \pm 1.51$ \\    
%     $\rho_{1} (10^{-3})$ 
%     & $<2.786$ & $<2.661$ & $<3.112$ & $<2.483$\\
%     $\rho_{2} (10^{-3})$ 
%     & $<2.075$ & $<2.017$ & $<2.051$ & $1.454 \pm 0.286$\\ 
%     $q_{f,I}$ 
%     & $0.027 \pm 0.005 $ & $0.023 \pm 0.004 $ & $0.027 \pm 0.005 $ & $0.014 \pm 0.003 $ \\  
%     $q_{f,V}$  
%     & $0.020 \pm 0.005 $ & $0.008 \pm 0.002 $ & $0.023 \pm 0.005 $ & $0.005 \pm 0.001 $\\ 
%     $q_{f,r}$ 
%     & $0.027 \pm 0.006 $ & $0.024 \pm 0.005 $ & $0.026 \pm 0.005 $ & $0.008 \pm 0.002 $ \\ 
%     $I_{\rm S1, OGLE}$ 
%     & $20.222 \pm 0.041$ & $20.203 \pm 0.039$ & $20.221 \pm 0.041$ & $20.207 \pm 0.047$\\
    
%     $V_{\rm S1, OGLE}$
%     & $22.021 \pm 0.041$ & $21.979 \pm 0.040$ & $22.025 \pm 0.041$ & $21.993 \pm 0.054$\\
    
%     $I_{\rm S2, OGLE}$
%     & $24.185 \pm 0.213$ & $24.303 \pm 0.200$ & $24.159 \pm 0.182$ & $24.912 \pm 0.257$\\
    
%     $V_{\rm S2, OGLE}$ 
%     & $26.288 \pm 0.269$ & $27.203 \pm 0.259$ & $26.156 \pm 0.215$ & $27.845 \pm 0.323$\\
    
%     $I_{\rm B, OGLE}$ 
%     & $18.231 \pm 0.052$ & $18.234 \pm 0.052$ & $18.231 \pm 0.052$ & $18.231 \pm 0.052$\\
    
%     $V_{\rm B, OGLE}$ 
%     & $19.996 \pm 0.103$ & $20.001 \pm 0.103$ & $19.996 \pm 0.103$ & $19.998 \pm 0.103$\\

%     \hline
%     $\chi^2_{\rm color}$ & ... & ... & $0.12$ & $0.04$\\
%     $(V - I)_{S2}$ 
%     &  $2.10 \pm 0.13 $ &  $2.90 \pm 0.09$ &  $2.00 \pm 0.09 $ &  $2.93 \pm 0.12$\\
%     \hline
%     \hline
%     \end{tabular}
%     \begin{tablenotes}
%         \centering
%         \item{NOTE. } ${\rm HJD}^{\prime} = {\rm HJD} - 2450000$. 
%         The upper limits on $\rho_{1}$ and $\rho_{2}$ are $3\sigma$.
%         %The $3\sigma$ upper limits of the non-detection parameters are reported instead.
%     \end{tablenotes}
%     %\tablecomments{The upper limits on $\rho$ are at $3\sigma$.}
%     \label{parm_1L2S}
% \end{table*}

% \begin{figure*}%[htbp]
%   \centering

%   \begin{subfigure}{0.33\textwidth}
%     \includegraphics[width=\textwidth]{Fig/KB220954_1L2S_grid.pdf}
%     \caption{KMT-2022-BLG-0954}
%     \label{fig:sub1}
%   \end{subfigure}
%   \hfill
%   \hspace{0.01\textwidth}
  
%   \begin{subfigure}{0.33\textwidth}
%     \includegraphics[width=\textwidth]{Fig/KB240697_1L2S_grid.pdf}
%     \caption{KMT-2024-BLG-0697}
%     \label{fig:sub2}
%   \end{subfigure}
%   \hfill
%   \hspace{0.01\textwidth}
  
%   \begin{subfigure}{0.33\textwidth}
%     \includegraphics[width=\textwidth]{Fig/KB220954_1L2S_grid.pdf}
%     \caption{KMT-2024-BLG-1170}
%     \label{fig:sub3}
%   \end{subfigure}
%   % \hfill
%   \hspace{1\textwidth}

%   \caption{1L2S grid search for three events}
%   \label{1L2S_grid}
% \end{figure*}



\begin{figure*}
  \centering

  \begin{minipage}{0.33\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Fig/KB220954_1L2S_grid.pdf}
    
    \vspace{0.5em}
    \parbox{0.9\textwidth}{\centering (a) KMT-2022-BLG-0954}
  \end{minipage}
  \hfill
  \begin{minipage}{0.33\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Fig/KB240697_1L2S_grid.pdf}
    
    \vspace{0.5em}
    \parbox{0.9\textwidth}{\centering (b) KMT-2024-BLG-0697}
  \end{minipage}
  \hfill
  \begin{minipage}{0.33\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Fig/KB241170_1L2S_grid.pdf}
    
    \vspace{0.5em}
    \parbox{0.9\textwidth}{\centering (c) \eventc}
  \end{minipage}

  \caption{1L2S grid search for three events. with respect to the best 2L1S solutions. For xxx, the best 2L1S solutions are Binary DA... , respectively. }
  \label{1L2S_grid}
\end{figure*}

% \begin{table*}
%     \caption{Physical parameters from Bayesian analysis for the three events}
%     \renewcommand{\arraystretch}{1.4}
%     \centering
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     %%%% the following is with 'Relative Weights'
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     % \begin{tabular}{c c ccccccc  c  c c}
%     % \hline\hline

    
%     % \multirow{2}{*}{Event} & \multirow{2}{*}{Model} 
%     % & \multicolumn{7}{c}{Physical Properties} &  & \multicolumn{2}{c}{Relative Weights} & \cline{3-9} 
%     % \cline{11-12} %\\
    
%     %   & & $D_{\rm S}$ (kpc) & $D_{\rm L}$ (kpc) & $M_{\rm primary}$  & $M_{\rm secondary}$  & $r_{\perp}$ (au) & $\mu_{\rm hel, rel}$ (${\rm mas\,yr^{-1}}$) & $\pi_{\rm E}$ & & Gal. Mod. & $\chi^2$ \\ \hline 

%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     %%%% the following is without 'Relative Weights'
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{c c ccccccc}
%     \hline\hline

    
%     \multirow{2}{*}{Event} & \multirow{2}{*}{Model} 
%     & \multicolumn{7}{c}{Physical Properties}  & \cline{3-9} 
%      %\\
    
%       & & $D_{\rm S}$ (kpc) & $D_{\rm L}$ (kpc) & $M_{\rm primary}$  & $M_{\rm secondary}$  & $r_{\perp}$ (au) & $\mu_{\rm hel, rel}$ (${\rm mas\,yr^{-1}}$) & $\pi_{\rm E}$ \\ \hline 

      
%     KMT-2022-BLG-0954 
%     & Planet No FSE Close & $8.8^{+2.1}_{-1.0}$ & $6.3^{+1.4}_{-2.9}$ 
%     & $0.57^{+0.37}_{-0.30}$ $M_{\odot}$ & $0.72^{+0.53}_{-0.39}$ $M_{\rm Jup}$ & $1.2^{+0.5}_{-0.4}$ & $3.98^{+3.05}_{-1.56}$ & $0.11^{+0.13}_{-0.04}$ \\
    
%     & Planet No FSE Wide & $8.8^{+2.1}_{-1.0}$ & $6.3^{+1.4}_{-2.9}$
%     & $0.56^{+0.37}_{-0.30}$ $M_{\odot}$ & $0.75^{+0.56}_{-0.41}$ $M_{\rm Jup}$ & $6.3^{+2.4}_{-2.2}$ & $3.96^{+3.03}_{-1.55}$ & $0.11^{+0.13}_{-0.04}$ \\ 
    
%     & Binary D→A Close & $8.8^{+2.0}_{-1.0}$ & $6.5^{+1.3}_{-2.9}$ & $0.55^{+0.37}_{-0.30}$ $M_{\odot}$ & $80.58^{+80.11}_{-50.84}$ $M_{\rm Jup}$ & $0.3^{+0.1}_{-0.1}$ & $4.09^{+2.97}_{-1.58}$ & $0.10^{+0.11}_{-0.04}$ \\
    
%     & Binary D→A Wide & $8.8^{+2.1}_{-1.0}$ & $6.5^{+1.3}_{-3.0}$ & $0.56^{+0.37}_{-0.30}$ $M_{\odot}$ & $106.79^{+109.17}_{-68.43}$ $M_{\rm Jup}$ & $40.7^{+18.3}_{-15.0}$ & $3.84^{+2.94}_{-1.51}$ & $0.10^{+0.11}_{-0.04}$ \\ 
%     \hline




%     KMT-2024-BLG-0697 
%      & Planet Close & $8.5^{+1.3}_{-0.8}$ & $7.1^{+0.7}_{-0.8}$ & $0.31^{+0.27}_{-0.16}$ $M_{\odot}$ & $0.77^{+0.68}_{-0.40}$ $M_{\rm Jup}$ & $1.1^{+0.2}_{-0.2}$ & $5.97^{+0.90}_{-0.83}$ & $0.10^{+0.10}_{-0.04}$ \\
     
%      & Planet Wide & $8.5^{+1.3}_{-0.8}$ & $7.2^{+0.7}_{-0.8}$ & $0.31^{+0.27}_{-0.16}$ $M_{\odot}$ & $0.77^{+0.68}_{-0.40}$ $M_{\rm Jup}$ & $2.7^{+0.4}_{-0.4}$ & $5.90^{+0.89}_{-0.82}$ & $0.10^{+0.09}_{-0.04}$ \\
     
%      & Binary A→B Close & $8.5^{+1.2}_{-0.8}$ & $7.0^{+0.7}_{-0.9}$ & $0.36^{+0.28}_{-0.18}$ $M_{\odot}$ & $17.73^{+15.52}_{-9.48}$ $M_{\rm Jup}$ & $0.4^{+0.1}_{-0.1}$ & $7.09^{+1.17}_{-1.07}$ & $0.09^{+0.09}_{-0.04}$ \\
     
%      & Binary A→B Wide & $8.5^{+1.2}_{-0.8}$ & $7.0^{+0.7}_{-0.9}$ & $0.36^{+0.28}_{-0.18}$ $M_{\odot}$ & $19.31^{+17.31}_{-10.41}$ $M_{\rm Jup}$ & $9.8^{+1.9}_{-1.9}$ & $6.93^{+1.14}_{-1.05}$ & $0.09^{+0.09}_{-0.04}$ \\ 
%      \hline

%      KMT-2024-BLG-1170 
%      & Planet Close & $9.7^{+0.9}_{-1.0}$ & $8.0^{+0.9}_{-1.5}$ & $0.31^{+0.32}_{-0.19}$ $M_{\odot}$ & $1.88^{+2.01}_{-1.17}$ $M_{\rm Jup}$ & $1.2^{+0.5}_{-0.4}$ & $6.21^{+2.68}_{-2.23}$ & $0.09^{+0.11}_{-0.04}$ \\
     
%      & Planet Wide & $9.7^{+0.9}_{-1.0}$ & $8.0^{+0.9}_{-1.5}$ & $0.30^{+0.32}_{-0.19}$ $M_{\odot}$ & $1.92^{+2.06}_{-1.19}$ $M_{\rm Jup}$ & $2.5^{+1.0}_{-0.9}$ & $6.16^{+2.67}_{-2.20}$ & $0.09^{+0.11}_{-0.04}$ \\
     
%      & Binary C→D Close & $9.6^{+0.9}_{-0.9}$ & $8.1^{+0.9}_{-1.2}$ & $0.22^{+0.28}_{-0.13}$ $M_{\odot}$ & $0.13^{+0.17}_{-0.08}$ $M_{\odot}$ & $0.4^{+0.2}_{-0.1}$ & $6.76^{+2.79}_{-2.29}$ & $0.08^{+0.09}_{-0.04}$ \\
     
%      & Binary C→D Wide & $9.7^{+1.0}_{-1.1}$ & $7.6^{+1.1}_{-2.4}$ & $0.11^{+0.11}_{-0.07}$ $M_{\odot}$ & $0.44^{+0.36}_{-0.26}$ $M_{\odot}$ & $21.3^{+7.8}_{-6.9}$ & $5.27^{+2.55}_{-1.76}$ & $0.08^{+0.10}_{-0.03}$ \\
     
%     %Combined & $0.61_{-0.33}^{+0.42}$ & $16.90_{-9.21}^{+12.90}$ & $3.3_{-1.8}^{+1.5}$ & $5.1_{-2.4}^{+1.9}$ & $7.8_{-1.4}^{+1.9}$ \\  
%      \hline \hline
%     \end{tabular}
%     }% this right bracket is for '\resizebox{\textwidth}{!}{'
    
%     \begin{tablenotes}
%         \centering
%       %\item[1] $P_{\rm disk}$ is the probability of a lens in the Galactic disk.
%     \end{tablenotes}
%     \label{table:bayes}
% \end{table*}







% \begin{table*}
%     \caption{Physical parameters from Bayesian analysis for \eventa}
%     \renewcommand{\arraystretch}{1.4}
%     \centering
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     %%%% the following is with 'Relative Weights'
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     % \begin{tabular}{c ccccccc  c  c c}
%     % \hline\hline

    
%     % \multirow{2}{*}{Event} & 
%     % \multirow{2}{*}{Model} 
%     % & \multicolumn{7}{c}{Physical Properties} &  & \multicolumn{2}{c}{Relative Weights} & \cline{2-8} 
%     % \cline{10-11} %\\
    
%     %   & & $D_{\rm S}$ (kpc) & $D_{\rm L}$ (kpc) & $M_{\rm primary}$  & $M_{\rm secondary}$  & $r_{\perp}$ (au) & $\mu_{\rm hel, rel}$ (${\rm mas\,yr^{-1}}$) & $\pi_{\rm E}$ & & Gal. Mod. & $\chi^2$ \\ \hline 

%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     %%%% the following is without 'Relative Weights'
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{c c ccccccc}
%     \hline\hline

    
%     \multirow{2}{*}{Event} & \multirow{2}{*}{Model} 
%     & \multicolumn{7}{c}{Physical Properties}  & \cline{3-9} 
%      %\\
    
%       & & $D_{\rm S}$ (kpc) & $D_{\rm L}$ (kpc) & $M_{\rm primary}$  & $M_{\rm secondary}$  & $r_{\perp}$ (au) & $\mu_{\rm hel, rel}$ (${\rm mas\,yr^{-1}}$) & $\pi_{\rm E}$ \\ \hline 

      
%     KMT-2022-BLG-0954 
%     & Planet No FSE Close & $8.8^{+2.1}_{-1.0}$ & $6.3^{+1.4}_{-2.9}$ 
%     & $0.57^{+0.37}_{-0.30}$ $M_{\odot}$ & $0.72^{+0.53}_{-0.39}$ $M_{\rm Jup}$ & $1.2^{+0.5}_{-0.4}$ & $3.98^{+3.05}_{-1.56}$ & $0.11^{+0.13}_{-0.04}$ \\
    
%     & Planet No FSE Wide & $8.8^{+2.1}_{-1.0}$ & $6.3^{+1.4}_{-2.9}$
%     & $0.56^{+0.37}_{-0.30}$ $M_{\odot}$ & $0.75^{+0.56}_{-0.41}$ $M_{\rm Jup}$ & $6.3^{+2.4}_{-2.2}$ & $3.96^{+3.03}_{-1.55}$ & $0.11^{+0.13}_{-0.04}$ \\ 
    
%     & Binary D→A Close & $8.8^{+2.0}_{-1.0}$ & $6.5^{+1.3}_{-2.9}$ & $0.55^{+0.37}_{-0.30}$ $M_{\odot}$ & $80.58^{+80.11}_{-50.84}$ $M_{\rm Jup}$ & $0.3^{+0.1}_{-0.1}$ & $4.09^{+2.97}_{-1.58}$ & $0.10^{+0.11}_{-0.04}$ \\
    
%     & Binary D→A Wide & $8.8^{+2.1}_{-1.0}$ & $6.5^{+1.3}_{-3.0}$ & $0.56^{+0.37}_{-0.30}$ $M_{\odot}$ & $106.79^{+109.17}_{-68.43}$ $M_{\rm Jup}$ & $40.7^{+18.3}_{-15.0}$ & $3.84^{+2.94}_{-1.51}$ & $0.10^{+0.11}_{-0.04}$ \\ 
%     \hline




%     KMT-2024-BLG-0697 
%      & Planet Close & $8.5^{+1.3}_{-0.8}$ & $7.1^{+0.7}_{-0.8}$ & $0.31^{+0.27}_{-0.16}$ $M_{\odot}$ & $0.77^{+0.68}_{-0.40}$ $M_{\rm Jup}$ & $1.1^{+0.2}_{-0.2}$ & $5.97^{+0.90}_{-0.83}$ & $0.10^{+0.10}_{-0.04}$ \\
     
%      & Planet Wide & $8.5^{+1.3}_{-0.8}$ & $7.2^{+0.7}_{-0.8}$ & $0.31^{+0.27}_{-0.16}$ $M_{\odot}$ & $0.77^{+0.68}_{-0.40}$ $M_{\rm Jup}$ & $2.7^{+0.4}_{-0.4}$ & $5.90^{+0.89}_{-0.82}$ & $0.10^{+0.09}_{-0.04}$ \\
     
%      & Binary A→B Close & $8.5^{+1.2}_{-0.8}$ & $7.0^{+0.7}_{-0.9}$ & $0.36^{+0.28}_{-0.18}$ $M_{\odot}$ & $17.73^{+15.52}_{-9.48}$ $M_{\rm Jup}$ & $0.4^{+0.1}_{-0.1}$ & $7.09^{+1.17}_{-1.07}$ & $0.09^{+0.09}_{-0.04}$ \\
     
%      & Binary A→B Wide & $8.5^{+1.2}_{-0.8}$ & $7.0^{+0.7}_{-0.9}$ & $0.36^{+0.28}_{-0.18}$ $M_{\odot}$ & $19.31^{+17.31}_{-10.41}$ $M_{\rm Jup}$ & $9.8^{+1.9}_{-1.9}$ & $6.93^{+1.14}_{-1.05}$ & $0.09^{+0.09}_{-0.04}$ \\ 
%      \hline

%      KMT-2024-BLG-1170 
%      & Planet Close & $9.7^{+0.9}_{-1.0}$ & $8.0^{+0.9}_{-1.5}$ & $0.31^{+0.32}_{-0.19}$ $M_{\odot}$ & $1.88^{+2.01}_{-1.17}$ $M_{\rm Jup}$ & $1.2^{+0.5}_{-0.4}$ & $6.21^{+2.68}_{-2.23}$ & $0.09^{+0.11}_{-0.04}$ \\
     
%      & Planet Wide & $9.7^{+0.9}_{-1.0}$ & $8.0^{+0.9}_{-1.5}$ & $0.30^{+0.32}_{-0.19}$ $M_{\odot}$ & $1.92^{+2.06}_{-1.19}$ $M_{\rm Jup}$ & $2.5^{+1.0}_{-0.9}$ & $6.16^{+2.67}_{-2.20}$ & $0.09^{+0.11}_{-0.04}$ \\
     
%      & Binary C→D Close & $9.6^{+0.9}_{-0.9}$ & $8.1^{+0.9}_{-1.2}$ & $0.22^{+0.28}_{-0.13}$ $M_{\odot}$ & $0.13^{+0.17}_{-0.08}$ $M_{\odot}$ & $0.4^{+0.2}_{-0.1}$ & $6.76^{+2.79}_{-2.29}$ & $0.08^{+0.09}_{-0.04}$ \\
     
%      & Binary C→D Wide & $9.7^{+1.0}_{-1.1}$ & $7.6^{+1.1}_{-2.4}$ & $0.11^{+0.11}_{-0.07}$ $M_{\odot}$ & $0.44^{+0.36}_{-0.26}$ $M_{\odot}$ & $21.3^{+7.8}_{-6.9}$ & $5.27^{+2.55}_{-1.76}$ & $0.08^{+0.10}_{-0.03}$ \\
     
%     %Combined & $0.61_{-0.33}^{+0.42}$ & $16.90_{-9.21}^{+12.90}$ & $3.3_{-1.8}^{+1.5}$ & $5.1_{-2.4}^{+1.9}$ & $7.8_{-1.4}^{+1.9}$ \\  
%      \hline \hline
%     \end{tabular}
%     }% this right bracket is for '\resizebox{\textwidth}{!}{'
    
%     \begin{tablenotes}
%         \centering
%       %\item[1] $P_{\rm disk}$ is the probability of a lens in the Galactic disk.
%     \end{tablenotes}
%     \label{table:bayes}
% \end{table*}




% \begin{figure*}
%     \centering
%     \includegraphics[width=0.33\textwidth]{Fig/KB220954_1L2S_grid.pdf}
%     \includegraphics[width=0.33\textwidth]{Fig/KB240697_1L2S_grid.pdf}
%     \includegraphics[width=0.33\textwidth]{Fig/KB220954_1L2S_grid.pdf}
%     \caption{1L2S grid search for three events. with respect to the best 2L1S solutions. For xxx, the best 2L1S solutions are Binary DA... , respectively. }
% \label{1L2S_grid}
% \end{figure*}

The ``Planet/Binary'' degeneracy is both scientifically important and frequently encountered in observations. 
As emphasized by \citet{Sean2022}, it is likely the most important degeneracy for exoplanet demographics, since interpreting an event as a planetary system or a stellar binary system has a direct impact on exoplanet statistics. 
The prevalence of this degeneracy was first noted by \citet{OB110950}, who pointed out that even within a single season, multiple events exhibited this ambiguity, suggesting that this degeneracy is common. 

In addition, as noted in Section~\ref{intro}, three events with this degeneracy were excluded from the 63-planet sample of the KMTNet for the mass-ratio function analysis, reducing the sample by 5\%. 
Consistent with this, our follow-up program since July 2020 has identified several dozen anomalous microlensing events, among which four are subject to the ``Planet/Binary'' degeneracy, including the three events analyzed in this work and KMT-2025-BLG-1314 (Ren et al., in preparation). 
This frequency reinforces its importance for exoplanet statistics, as events affected by this degeneracy can constitute a non-negligible fraction of the total sample. 


% 1. the importance and common of this degeneracy: 
% Sean 2022 
% "This particular case is the most important type of degeneracy for exoplanet demographics, because the distinction between a planetary mass or stellar binary companion has direct consequences for microlensing exoplanet statistics."
% "this degeneracy is likely the most important of its kind when it comes to exoplanet demographics, because the ambiguity of the lens system parameters from the light curve modeling have a direct consequence on the exoplanet statistics that are drawn from the data (i.e. planetary systems vs. non-planetary systems)."

% common: 4/several dozens in follow-up; choi 2012, two events in the same year

 
% All three events analyzed in this work do not break the ``Planet/Binary'' degeneracy (through modeling the light curve and comparing the goodness of fit/from the light-curve analysis). 
% Table \ref{historyevents} summarizes known events subject to the ``Planet/Binary'' degeneracy and $\Delta\chi^2$ between the best-fit binary and planet model for each event. 
% All (but one) events have $|\Delta\chi^2|<\sim25$, thus the degeneracy cannot be broken at the $>5\sigma$ level, indicating this degeneracy is very severe. 
% The only exception is OGLE-2015-BLG-1212 \citep{Bozza2016}, which is observed by both ground-based telescopes and textit{Spitzer}. 
% Observing the event from a satellite introduces a second source trajectory that probes a different part of the magnification pattern, thus helping break the ``Planet/Binary'' degeneracy as degenerate magnification pattern on both source trajectories is much harder. 
% However, the next generation space-based microlensing telescopes like \textit{Roman}\footnote{https://roman.gsfc.nasa.gov/} and {Earth 2.0}\footnote{https://et.shao.ac.cn/} which will orbit the Sun-Earch L2 point have much shorter (Earth-satellite projected separation/baseline) than \textit{Spitzer} (i.e., $\sim0.01 \rm au$ compared to $\sim1 \rm au$), leading to much smaller differences between two source trajectories, thus making breaking the degeneracy through satellite parallax effect even harder. 
% A targeted work on the satellite parallax effect for the next generation space-based microlensing telescopes orbiting the Sun-Earch L2 point will be presented (separately/elsewhere). 

% 2. all three events cannot be broken by lc, and history events also cannot break by lc dchi2, see Table \ref{historyevents}

A similar situation applies to MOA-2015-BLG-337 and OGLE-2018-BLG-1554, where the planet model predicts slow and well-constrained $\murel$, while the binary model leaves $\murel$ essentially unconstrained. 
In such cases, if the directly measured $\murel$ significantly deviates from the prediction of the planet model, the planet interpretation can be excluded. 
A more complex case is presented by \eventa, which admits both a ``Planet Finite'' model that provides precise and low $\murel$ estimates and a ``Planet Point'' model for which $\murel$ is unmeasurable. 
As a result, even if future high-resolution imaging rejects the ``Planet Finite'' model based on a mismatch in $\murel$, the degeneracy will persist due to the viable ``Planet Point'' model. 

OGLE-2012-BLG-0455 and \eventb represent a different scenario in which both the binary and planet models yield measurable $\murel$, but with large uncertainties that result in nearly overlapping $1\sigma$ ranges. 
In such circumstances, a direct measurement of $\murel$ that falls within the overlap fails to resolve the degeneracy, whereas a value well above or below this range could favor one model over the other. 
By contrast, for \eventc and other events where $\murel$ is unmeasurable for both models, the degeneracy remains entirely unresolved. 

==> changelog.tex <==
250911,jiyuan:

update 220954 2L1S parameter table with limb, 
update 220954 lc figure with limb,

Equation (59) --> Equation (60) and (61)
because Equation (59) only works at small q, and differs significantly from the true boundary at large q; 
while Equation (60) and (61) is the true boundary at all q ranges
(Equation (3) and (4) of \citet{Cassan2008} is the same as Equation (60) and (61) of Dominik (1999))

2 places in Section 3.2

Table 220954 cmd

Table 1L2S and text 1L2S

Table 12

bayes of kb220954 is rerun, table is updated for param, dchi2 ga and dchi2 lc

bayes text updated
